Adaptive Diffusions for Scalable Learning over Graphs

Diffusion-based classifiers such as those relying on the Personalized PageRank and the Heat kernel, enjoy remarkable classification accuracy at modest computational requirements. Their performance however is affected by the extent to which the chosen diffusion captures a typically unknown label propagation mechanism, that can be specific to the underlying graph, and potentially different for each class. The present work introduces a disciplined, data-efficient approach to learning class-specific diffusion functions adapted to the underlying network topology. The novel learning approach leverages the notion of "landing probabilities" of class-specific random walks, which can be computed efficiently, thereby ensuring scalability to large graphs. This is supported by rigorous analysis of the properties of the model as well as the proposed algorithms. Furthermore, a robust version of the classifier facilitates learning even in noisy environments. Classification tests on real networks demonstrate that adapting the diffusion function to the given graph and observed labels, significantly improves the performance over fixed diffusions; reaching -- and many times surpassing -- the classification accuracy of computationally heavier state-of-the-art competing methods, that rely on node embeddings and deep neural networks.

==> figs/matlab2tikz-matlab2tikz-816f875/test/template/Makefile <==
# ./Makefile

ECHOCMD:=/bin/echo -e
LATEX:=pdflatex --shell-escape
TARGET:=acid

main:
	cd data/reference/ && $(MAKE)
	cd data/converted/ && $(MAKE)
	@$(LATEX) $(TARGET)

.PHONY: clean

clean:
	@rm -f $(TARGET).aux \
	$(TARGET).log \
	$(TARGET).nav \
	$(TARGET).out \
	$(TARGET).snm \
	$(TARGET).toc \
	$(TARGET).vrb \
	$(TARGET).pdf \
	$(TARGET).dvi \
	$(TARGET).ps \
	missfont.log
	@rm -f *~
	cd data/reference/ && $(MAKE) clean
	cd data/converted/ && $(MAKE) clean

distclean: clean
	@rm -f $(TARGET).tex
	cd data/reference/ && $(MAKE) distclean
	cd data/converted/ && $(MAKE) distclean


==> figs/matlab2tikz-matlab2tikz-816f875/test/template/data/converted/Makefile <==
# ./Makefile

ECHOCMD:=/bin/echo -e
LATEX:=pdflatex --shell-escape -interaction=batchmode

TEST_SRCS:=$(wildcard test*-converted.tex)
TEST_PDFS:=$(TEST_SRCS:.tex=.pdf)

default: $(TEST_PDFS)

%.pdf: %.tex
	@$(LATEX) $<

.PHONY: clean

clean:
	rm -f test*-converted.aux \
		test*-converted.log \
		test*-converted.pdf

distclean: clean
	rm -f test*-converted.tex \
		test*-converted*.png

